A Receding Horizon Push Recovery Strategy for Balancing the iCub Humanoid Robot

Balancing and reacting to strong and unexpected pushes is a critical requirement for humanoid robots. We recently designed a capture point based approach which interfaces with a momentum-based torque controller and we implemented and validated it on the iCub humanoid robot. In this work we implement a Receding Horizon control, also known as Model Predictive Control, to add the possibility to predict the future evolution of the robot, especially the constraints switching given by the hybrid nature of the system. We prove that the proposed MPC extension makes the step-recovery controller more robust and reliable when executing the recovery strategy. Experiments in simulation show the results of the proposed approach.

==> tex/qp.tex <==
%!TEX root = ../steprecovery.tex
\section{Quadratic Programming Transcription} \label{sec:qp}

We solve the finite-horizon Optimal Control problem presented in the previous section by using numerical methods. In particular we convert the original optimal control problem into a Quadratic Programming problem.
It is therefore necessary to discretize the problem and to reformulate it so as to fit the problem into a Quadratic Programming (QP) formulation and subsequently solve it by using state-of-the-art QP solvers.

The general form of a QP problem is the following:
\begin{IEEEeqnarray}{CRCL}
	\IEEEyesnumber \phantomsection \label{c6eq:optim}
	\minimize_\chi& \frac{1}{2}\chi^\top H \chi &+& \chi^\top \mathbbm{g} \IEEEyessubnumber \label{c6eq:optim_cost}\\ 
	\text{subject to:} & A^{leq}\chi &\leq& b^{leq} \IEEEyessubnumber
\end{IEEEeqnarray}
where $\chi$ is the optimization variable, $H$ a positive semi-definite matrix (the ``Hessian'' matrix), $\mathbbm{g}$ the ``gradient'' vector, while $A^{eq}$, $b^{eq}$, $A^{leq}$, $b^{leq}$ are the terms expressing the equality and inequality constraints respectively.

\subsection{Model Transcription}

We discretize the model using forward Euler formulation. Different approaches may have been chosen, as described in \cite{BettsPractical2010}, but this is the most suitable for our application thanks to its simplicity. Hence, the continuous dynamical system in Eq. \eqref{c6eq:genmodel} can be discretized into the following discrete-time system:
\begin{equation}
\begin{split}
&x(k+1) = x(k) + \mathrm{f}(x(k),u(k))\dif t\\
&k = 0, 1, \cdots\, , \, N-1 
\end{split}
\end{equation} 
where $k \in \mathbb{N}$ is the discrete time, $N=\ceil{t_f/\mathrm{d}t}$ and $\dif t\in \mathbb{R}$ is the time step length.

Consider Eq. \eqref{c6eq:model}, its discretization is:
\begin{equation}\label{c6eq:discrmodel}
\gamma(k+1) = Ev_\gamma \gamma(k) + F_\gamma f(k) +G_\gamma + S_\gamma ^0
\end{equation}
where
\begin{equation*}
Ev_\gamma = 1_9 + \mathrm{d}t\tilde{E}v_\gamma,\, F_\gamma = \mathrm{d}t\tilde{F}_\gamma, \, G_\gamma = \mathrm{d}t\tilde{g}_\gamma, \, S_\gamma ^0 = \mathrm{d}t\tilde{S}^0_\gamma.
\end{equation*}

We can now define the optimization vector $\chi$ as the collection of all the states and control variables over the horizon. Formally:
\begin{equation}
\chi =
\begin{bmatrix}
\gamma(1)\\
f(0)\\
\vdots\\
\gamma(k)\\
f(k-1)\\
\vdots\\
\gamma(N)\\
f(N-1)
\end{bmatrix}, \: \chi \in \mathbb{R}^{9N+12N}.
\end{equation}
According to the receding horizon principle, at each time step, $f(0)$ will be applied to the system, through the balancing controller already implemented on iCub, as presented in Sec. \ref{sec:model}. In fact, the first task controls the CoM through the definition of desired wrenches.

A crucial point to be considered, is the definition of the time instant at which the impact occurs.
We assume the impact to be impulsive and taking place at the beginning of a time step which we denote with $k_{impact}$.
We further assume that the control input $f(k)$ is applied, constantly, for the whole duration of the time step $k$, i.e. from $k$ to $k+1$. 
This implies that the computation time is not taken into account in the dynamical model.
Since, at the current stage, we tested the presented framework only in simulation this does not constitute an issue. 
For a practical implementation on the real robot, we will address the aforementioned problem, e.g. we will model a one step delay for the application of the control action.
Note that, in view of the above two assumptions, setting $k_{impact} = 0$ implies that both feet are at contact already at the initial time $k = 0$.

As mentioned previously, we do not directly model the distance between the swing foot and the ground, but we compute the position and the expected impact time at the beginning of the push strategy.
The following procedure describes how we update the expected impact instance throughout the proposed MPC controller.
Assuming the initial time instant to be always set to zero, we decrement the $k_{impact}$ by one at each controller execution.
If the impact has not occurred yet, we saturate, from below, $k_{impact}$ to $1$, i.e. we expect the impact to occur at the second time step.
If the impact has occurred, instead, $k_{impact}$ is correctly set to $0$.
The definition of the impact time and the trajectory control of mechanical system with unilateral constraints (as it is our case), are still an open research problem \cite{rijnen2015optimal,biemond2013tracking}. 

%\begin{figure}[t]
%	\centering 
%	\def\svgwidth{0.9\columnwidth}
%	\import{images/}{timescale2.pdf_tex}
%	\caption{The upper time-line shows the feedback and the prediction for the state. At each time instant, $\gamma$ is either obtained by feedback $\left(\gamma(0)\right)$ or by prediction (from $\gamma(1)$ on). Between two subsequent time steps, the desired wrench is computed. E.g., $f(0)$ is computed between 0 and 1 and applied between 1 and 2. Thus, the second time-line illustrates when the desired wrenches are applied and, below, whether only one or two feet are employed. The impact is expected to be in 2 (i.e. $k_{impact} = 2$) therefore $f(1)$ will define a desired wrench even for the swing foot. As a consequence, by saturating $k_{impact}$ to 2, $f(0)$ will not include a desired wrench for the swing foot. On the other hand, when the impact is sensed by the robot, $k_{impact}$ can be constantly set to 1. }\label{c6im:timescale}
%\end{figure}

It is now possible to write the discretized dynamics as an equality constraints, transforming the initial continuous time optimal control problem of Eq. \eqref{c6eq:ocdef} into Eq. \eqref{c6eq:optim}. By expanding Eq. \eqref{c6eq:discrmodel} over the horizon we get the following constraint:
\begin{equation} \label{c6eq:qp_ev}
\left(Ev - e_\gamma\right) \chi = -G - Ev_{\gamma_0} - S^0
\end{equation}
where $Ev \in \mathbb{R}^{9N\times 21N}$ and $G, \:Ev_{\gamma_0}, \:S^0 \in \mathbb{R}^{9N\times 1}$. The matrix $e_\gamma\in\mathbb{R}^{9N\times 21N}$ selects the terms related to state $\gamma$ from vector $\chi$, namely:
\begin{equation*}
e_\gamma=
\begin{bmatrix}
1_9 & 0_{9\times 12} && \cdots && 0_{9\times 9} & 0_{9\times 12}\\
0_{9\times 9} & 0_{9\times 12} & 1_9 & 0_{9\times 12} & \cdots & 0_{9\times 9} & 0_{9\times 12} \\
\vdots&\vdots&&\ddots&&&\vdots\\
0_{9\times 9} & 0_{9\times 12} &&\cdots&&1_9 & 0_{9\times 12}
\end{bmatrix}.
\end{equation*}
$Ev$ has the following expression:
\begin{equation*}
\setlength{\arraycolsep}{3pt} 
\begin{split}
&Ev = \begin{bmatrix}
		0_{9\times 9} &  F_\gamma    & 0_{9\times 9}&0_{9\times 12}&\cdots&0_{9\times 12}\\
		0_{9\times 9} &0_{9\times 12}& 0_{9\times 9}&  F_\gamma  &\cdots &0_{9\times 12} \\
		\vdots& &\ddots&&\ddots&\\
		0_{9\times 9} &0_{9\times 12}&  \cdots   & &0_{9\times 9}&F_\gamma  
	\end{bmatrix}+\\
	&+ \begin{bmatrix}
		0_{9\times 9} &  0_{9\times 12}  &&\cdots& &&0_{9\times 9}&0_{9\times 12}\\
		Ev_\gamma &0_{9\times 12}& 0_{9\times 9}& 0_{9\times 12} &\cdots &&0_{9\times 9}&0_{9\times 12} \\
		0_{9\times 9} &0_{9\times 12}& Ev_\gamma& 0_{9\times 12} &\cdots &&0_{9\times 9}&0_{9\times 12} \\
		\vdots& &&\ddots&&\ddots&\vdots&\vdots\\
		0_{9\times 9} &0_{9\times 12}&\cdots&& Ev_\gamma   &0_{9\times 12} &0_{9\times 9}&0_{9\times 12} 
	\end{bmatrix}.
\end{split}
\end{equation*}
It is possible to notice that $\gamma(1)$ depends directly only on $\gamma(0)$, which is the feedback part of the state. This dependency is introduced through $Ev_{\gamma_0}$, which therefore has the following structure:
\begin{equation*}
Ev_{\gamma_0} = \begin{bmatrix}
Ev_\gamma\\
0_{9\times 9}\\
\vdots\\
0_{9\times 9}
\end{bmatrix}\gamma(0).
\end{equation*}
Finally $G$ considers the gravitational effects, while $S^0$ contains the constant terms related to the angular momentum:
\begin{equation*}
G = \begin{bmatrix}
G_\gamma\\
\vdots\\
G_\gamma
\end{bmatrix},\quad S^0 = \begin{bmatrix}
S^0_\gamma\\
\vdots\\
S^0_\gamma
\end{bmatrix}.
\end{equation*}

A similar approach can be used to transcribe the constraints presented in \ref{c6sec:constraints}, taking in mind their varying structure at the impact instant. We avoid here the full dissertation for the sake of conciseness.

%\subsection{Constraints Transcription}
%Now, it is possible to translate all the constraints defined in Sec. \ref{c6sec:constraints} as a function of the optimization variable $\chi$.
%
%\subsubsection{Constraints on the Left Foot Wrench}
%The constraints on the left foot do not change over the horizon since the left foot is supposed to be the stance foot. 
%The goal therefore is to write these constraints as
% \begin{equation}\label{c6eq:fl_discr}
% A_{hor, L}\: \chi \leq b_{hor, L}
% \end{equation}
% where $A_{hor, L}$ and $b_{hor, L}$ are basically a composition of matrices $A_{cl}$ and $b_{cl}$ introduced in Eq. \eqref{c6eq:wrench_constr}. 
% In particular:
% \begin{equation}
%      A_{hor, L}{=}\begin{bmatrix}
%     A_{cl} & 0_{ncl\times 6}& \cdots &0_{ncl\times 6}\\
%     0_{ncl\times 6} & A_{cl} &0_{ncl\times 6}& \cdots\\
%     \vdots& &\ddots& \\
%     0_{ncl\times 6}&\cdots& & A_{cl}
%     \end{bmatrix} E_{fl} E_f  \label{c6eq:EFdef}
% \end{equation}
% with
% \begin{equation*}
% E_{fl} = \begin{bmatrix}
%						\begin{bmatrix}{1}_6 & 0_{6\times 6}\end{bmatrix} &  0_{6\times12} & \cdots & 0_{6\times12}\\
%						0_{6\times12} & \begin{bmatrix}{1}_6 & 0_{6\times 6}\end{bmatrix} & 0_{6\times12} & \cdots\\ 
%						\vdots& &\ddots& \\
%						0_{ncl\times 6}&\cdots& & \begin{bmatrix}{1}_6 & 0_{6\times 6}\end{bmatrix}
%						\end{bmatrix}
%\end{equation*}
%\begin{equation*}				
%E_f =  \begin{bmatrix}
%	0_{12\times 9N} & {1}_{12} & 0_{12\times12} & \cdots & 0_{12\times12}\\
%	0_{12\times 9N} &  0_{12\times12} & {1}_{12}&\cdots & 0_{12\times12}\\
%	\vdots                 &  \vdots  & &\ddots   & \vdots\\
%	0_{12\times 9N} &  0_{12\times12} & \cdots & 0_{12\times12} & {1}_{12}
%\end{bmatrix}.
% \end{equation*}
%The first matrix from left replicates the constraints introduced in Eq. \eqref{c6eq:wrench_constr} over all the time instants in the horizon, having dimensions $ (n_{cl} N) \times 6N$ where $n_{cl}$ is basically equal to the number of rows of matrix $A_{cl}$. The second matrix, $E_{lf}$, extracts just the left wrench from the vector $\left[\begin{smallmatrix}
%f(0)  & f(1) & \cdots & f(N-1)\end{smallmatrix}\right]^\top $ obtained thanks to $E_f$, which therefore has dimensions $12N\times 21N$.
%
%Finally, $b_{hor, L}$ is the row-wise repetition of matrix $b_{cl}$, formally:
%\begin{equation*}
%b_{hor, L} = \begin{bmatrix}
%b_{cl}\\
%b_{cl}\\
%\vdots\\
%b_{cl}
%\end{bmatrix}  \in \mathbb{R}^{(n_{cl} \cdot N)}.
%\end{equation*}
% 
%\subsubsection{Constraints on the Right Foot Wrench} 
% The right foot is the swinging foot, therefore the constraints applied on the desired wrench are changing depending on the value of $k_{impact}$. In particular Eq. \eqref{c6eq:fr_cont_costr} can be rewritten as,
% \begin{equation}\label{c6eq:fr_discr_costr}
% \begin{cases}
% f_{r} = 0_6 &\forall k:\; 1 \leq k < k_{impact}\\
% A_{cr}f_r \leq b_{cr}  &\forall k:\; k_{impact} \leq k \leq N.
% \end{cases}
% \end{equation}
% We assume to have $1 < k_{impact} \leq N$, otherwise there will be just the first or the second set of constraints depending on whether the impact will happen over the horizon or it has already occurred, respectively. In general we will have two sets of constraints:
% \begin{IEEEeqnarray}{RCL}
% 	\IEEEyesnumber \phantomsection\label{c6eq:qp_fr}
% 	A^{eq}_{hor,R} \chi &=& b^{eq}_{hor,R} \IEEEyessubnumber\\
% 	A^{leq}_{hor,R} \chi &\leq& b^{leq}_{hor,R}. \IEEEyessubnumber \label{c6eq:fr_discr_leq}
% \end{IEEEeqnarray}
% The dimension of these matrices depends on the value of $k_{impact}$, but by virtue of the above, let us assume it to be inside the control horizon. The equality constraints would have the following form:
% \begin{equation}
%     \label{eq:constr_all_right}
%A^{eq}_{hor,R} = E^{eq}_{fr}  E^{eq}_f \in  \mathbb{R}^{6(k_{impact}-1)\times 21N}.
% \end{equation}
% The matrices $E^{eq}_{fr}$ and  $E^{eq}_f$ are responsible of selecting the right foot wrench from the optimization variable $\chi$ and are similar to the one reported in Eq. \eqref{c6eq:EFdef}.
% 
%% with
%% \begin{IEEEeqnarray*}{RCL}
%% \nonumber
%% E^{eq}_{fr} &=& \begin{bmatrix}
%% \begin{bmatrix}0_{6\times 6} & {1}_6\end{bmatrix} &  0_{6\times12} & \cdots & 0_{6\times12}\\
%% 0_{6\times12} & \begin{bmatrix}0_{6\times 6} & {1}_6\end{bmatrix} & 0_{6\times12} & \cdots\\
%% \vdots& &\ddots& \\
%% 0_{6\times 12}&\cdots& & \begin{bmatrix}0_{6\times 6} & {1}_6\end{bmatrix}
%% \end{bmatrix}\\
%% E^{eq}_f &=& \begin{bmatrix}
%%     0_{12\times 9N} & {1}_{12} & 0_{12\times12} & \cdots & 0_{12\times12} & 0_{12\times12} & \cdots & 0_{12\times12}\\
%%     0_{12\times 9N} &  0_{12\times12} & {1}_{12}&\cdots & 0_{12\times12} & 0_{12\times12}& \cdots & 0_{12\times12}\\
%%     \vdots                 &  \vdots  & &\ddots   & \vdots & \vdots &\ddots&\vdots\\
%%     0_{12\times 9N} &  0_{12\times12} & \cdots & 0_{12\times12} & {1}_{12} & 0_{12\times12}& \cdots & 0_{12\times12}
%% \end{bmatrix}
%% \end{IEEEeqnarray*}
%% where the matrix $E^{eq}_{fr} \in \mathbb{R}^{6(k_{impact}-1)\times 12(k_{impact}-1)}$ now extracts just the right wrench from the vector $\left[\begin{smallmatrix}
%% f(0)  & f(1) & \cdots & f(k_{impact}-2)\end{smallmatrix}\right]^\top $ obtained through $E^{eq}_f$ which therefore has dimension $12(k_{impact}-1) \times 21N$.
%
%Once the right wrenches of all the time steps before $k_{impact}$ has been extracted from vector $\chi$, they are set to zero thanks to matrix $b^{eq}_{hor,R} = 0_{6(k_{impact}-1)}$.
%
%For what concerns Eq. \eqref{c6eq:fr_discr_leq}, it will be structurally similar to Eq. \eqref{c6eq:fl_discr}, in fact:
%\begin{equation*}
%A^{leq}_{hor,R}=\underbrace{\begin{bmatrix}
%					A_{cr} & 0_{n_{cr}\times 6}& \cdots &0_{n_{cr}\times 6}\\
%					0_{n_{cr}\times 6} & A_{cr} &0_{n_{cr}\times 6}& \cdots\\
%					\vdots& &\ddots& \\
%					0_{n_{cr}\times 6}&\cdots& & A_{cr}
%				\end{bmatrix}}_{\in\: \mathbb{R}^{n_{cr} k_{2f}\times 6 k_{2f}}} E^{leq}_{fr}  E^{leq}_f	
%\end{equation*}
%with
%\begin{IEEEeqnarray*}{RCL}
%	k_{2f} &=& N-k_{impact}+1. %, \\[5pt]
%\end{IEEEeqnarray*}
%	% E^{leq}_f &=& \begin{bmatrix}
%%         0_{12\times 9N} & 0_{12\times12} & \cdots & 0_{12\times12} & {1}_{12} & 0_{12\times12} & \cdots & 0_{12\times12}\\
%%         0_{12\times 9B} & 0_{12\times12}& \cdots & 0_{12\times12}&  0_{12\times12} & {1}_{12}&\cdots & 0_{12\times12}\\
%%         \vdots                 & \vdots &\ddots&\vdots &  \vdots  & &\ddots   & \vdots \\
%%         0_{12\times 9N} & 0_{12\times12}& \cdots & 0_{12\times12} &  0_{12\times12} & \cdots & 0_{12\times12} & {1}_{12}
%%     \end{bmatrix}
%% \end{IEEEeqnarray*}
%while $E^{leq}_{fr}$ is structurally equal to $E^{eq}_{fr}$, but with dimensions $6k_{2f}\times 12k_{2f}$. 
%Here $n_{cr}$ is the number of rows of $A_{Cr}$ while $k_{2f}$ is the number of time steps in the horizon in which it is possible to use both feet for balancing.
%
%Finally,  
%\begin{equation*}
%b_{hor, R}^{leq} = \begin{bmatrix}
%b_{cr}\\
%b_{cr}\\
%\vdots\\
%b_{cr}
%\end{bmatrix} \in \mathbb{R}^{n_{cr}  k_{2f}}.
%\end{equation*}
%
%\subsubsection{Instantaneous Capture Point Constraints}
%The shape of these constraints is the following:
%\begin{equation}\label{c6eq:qp_icp}
%A_{hor, ch}\chi \leq b_{hor, ch}.
%\end{equation}
%
%Considering that we are dealing with a set of constraints involving only a subset of elements in $\chi$ (since they are enforced only after the impact event), the matrices describing the constraints will be obtained similarly as before.
%Indeed:
%\begin{equation*}
%A_{hor, ch} = \underbrace{\begin{bmatrix}
%	\begin{bmatrix}A_{ch} & 0_{nch}\end{bmatrix} &  \cdots &0_{nch\times 3}\\
%	\vdots& \ddots&\vdots \\
%	0_{nch\times 3}&\cdots&  \begin{bmatrix}A_{ch} & 0_{nch}\end{bmatrix}
%	\end{bmatrix}}_{\in\: \mathbb{R}^{nch\cdot k_{2f}\times 3k_{2f}}} E_{icp}  E^{k_{2f}}_\gamma
%\end{equation*}
%% \begin{equation*}
%% A_{hor, ch} = \underbrace{\begin{bmatrix}
%%     \begin{bmatrix}A_{ch} & 0_{nch}\end{bmatrix} & 0_{nch\times 3}& \cdots &0_{nch\times 3}\\
%%     0_{nch\times 3} & \begin{bmatrix}A_{ch} & 0_{nch}\end{bmatrix} &0_{nch\times 3}& \cdots\\
%%     \vdots& &\ddots& \\
%%     0_{nch\times 3}&\cdots& & \begin{bmatrix}A_{ch} & 0_{nch}\end{bmatrix}
%%     \end{bmatrix}}_{\in\: \mathbb{R}^{nch\cdot k_{2f}\times 3k_{2f}}}\cdot E_{icp} \cdot E^{k_{2f}}_\gamma
%% \end{equation*}
%with
%\begin{equation*}
%	E_{icp} = \begin{bmatrix}
%		\begin{bmatrix}{1}_3 & \frac{1}{\omega}{1}_3 & 0_{3\times 3}\end{bmatrix} &   \cdots & 0_{3\times9}\\
%		\vdots& \ddots& \vdots\\
%		0_{3\times 9}&\cdots& \begin{bmatrix}{1}_3 & \frac{1}{\omega}{1}_3 & 0_{3\times 3}\end{bmatrix}
%	\end{bmatrix},
%\end{equation*}
%% \begin{equation*}
%%     E_{icp} = \begin{bmatrix}
%%         \begin{bmatrix}{1}_3 & \frac{1}{\omega}{1}_3 & 0_{3\times 3}\end{bmatrix} &  0_{3\times9} & \cdots & 0_{3\times9}\\
%%         0_{3\times9} & \begin{bmatrix}{1}_3 & \frac{1}{\omega}{1}_3 & 0_{3\times 3}\end{bmatrix} & 0_{3\times9} & \cdots\\
%%         \vdots& &\ddots& \\
%%         0_{3\times 9}&\cdots& & \begin{bmatrix}{1}_3 & \frac{1}{\omega}{1}_3 & 0_{3\times 3}\end{bmatrix}
%%     \end{bmatrix},
%% \end{equation*}
%% \begin{equation*}
%% E^{k_{2f}}_\gamma = \begin{bmatrix}
%% 0_{9\times 9} & \cdots & 0_{9\times 9} & {1}_{9} & 0_{9\times 9} & \cdots & 0_{9\times 9}&0_{9\times 12N} \\
%% 0_{9\times 9}& \cdots & 0_{9\times 9}&  0_{9\times 9} & {1}_{9}&\cdots & 0_{9\times 9}&0_{9\times 12N}\\
%% \vdots&                 & \vdots &\vdots&  &  \ddots   &   & \vdots\\
%% 0_{9\times 9}& \cdots & 0_{9\times 9} &  0_{9\times 9} & \cdots & 0_{9\times 9} & {1}_{9}&0_{9\times 12N}
%% \end{bmatrix}.
%% \end{equation*}
%\begin{equation*}
%E^{k_{2f}}_\gamma = \begin{bmatrix}
%0_{9\times 9} & \cdots & 0_{9\times 9} & {1}_{9}  & \cdots & 0_{9\times 9}&0_{9\times 12N} \\
%\vdots&                 & \vdots &\vdots &  \ddots   &   & \vdots\\
%0_{9\times 9}& \cdots & 0_{9\times 9} &  0_{9\times 9} & \cdots  & {1}_{9} & 0_{9\times 12N} 
%\end{bmatrix}.
%\end{equation*}
%
%The first matrix repeat $A_{ch}$, as defined in Eq. \eqref{c6eq:icp_constr}, on the diagonal,  with an additional column that avoid considering the $z$ component of the ICP. 
%In fact, through matrix $E_{icp}$, the instantaneous capture point is computed using every $\gamma$ from $k_{impact}$ to $N$, avoiding considering just the angular momentum component available inside $\gamma$ (see its definition in Eq. \eqref{c6eq:gamma}). 
%Finally, matrix $E^{k_{2f}}_\gamma \in \mathbb{R}^{9k_{2f}\times 21N}$ extracts all the states $\gamma$ related to the time instants after the impact. 
%By coherence, here $n_{ch}$ is the number of rows of matrix $A_{ch}$. Finally, as usual, matrix $b_{hor, ch}$ is obtained by repetition of $b_{ch}$, namely
%\begin{equation*}
%b_{hor, ch} = \begin{bmatrix}
%b_{ch}\\
%b_{ch}\\
%\vdots\\
%b_{ch}
%\end{bmatrix}, \quad b_{hor, ch} \in \mathbb{R}^{n_{ch} k_{2f}}.
%\end{equation*}
%
%\subsection{Placing All Together}
%Now we can finally build-up the constraints matrices introduced in Eq. \eqref{c6eq:qp_ev}, \eqref{c6eq:fl_discr}, \eqref{c6eq:qp_fr} and \eqref{c6eq:qp_icp} into the constraints of Eq. \eqref{c6eq:optim}. In particular:
%\begin{IEEEeqnarray*}{RCLRCL}
%\phantomsection
%A^{eq} &=& \begin{bmatrix}
%Ev - \begin{bmatrix}
%{1}_{9N} & 0_{9N\times 12N}
%\end{bmatrix}\\[5pt]
%A^{eq}_{hor,R}
%\end{bmatrix}, & b^{eq} &=& \begin{bmatrix}
%							-G - Ev_{\gamma_0}\\[5pt]
%							b^{eq}_{hor,R}
%					     \end{bmatrix} \\[5pt]
%A^{leq} &=& \begin{bmatrix}
%		        A_{hor, L}\\[5pt]
%		        A^{leq}_{hor,R}\\[5pt]
%		        A_{hor, ch}	
%		  \end{bmatrix},	& b^{leq} &=& \begin{bmatrix}
%										  b_{hor, L}\\[5pt]
%										  b^{leq}_{hor,R}\\[5pt]
%										  b_{hor, ch}
%									 \end{bmatrix}		 
%\end{IEEEeqnarray*}
%generating therefore $9N + 6(k_{impact}-1)$ equality constraints and $n_{cl} N + (n_{cr}+n_{ch})(N-k_{impact}+1)$ inequality constraints.
%
\subsection{Cost Function Transcription}
The last stage of the transcription from a continuous optimal control problem to a QP formulation, involves the cost function of Eq. \eqref{c6eq:cost}. 
As before, this process consists in a discretization stage followed by a reformulation phase necessary to express the cost function in terms of $\chi$. This latter stage is omitted here, but it simply exploits the appropriate $e$ matrices, as it has been done for the model transcription.

Starting from the first term, Eq. \eqref{c6eq:cost_gamma}, the discretization corresponds to 
\begin{IEEEeqnarray}{C}
\IEEEyesnumber \phantomsection
\eqref{c6eq:cost_gamma} \Rightarrow \Gamma_\gamma = \frac{1}{2}\sum_{k=1}^{N} \norm {\gamma(k) - \gamma^d(k)}^2_{K_\gamma} 
\end{IEEEeqnarray}
noticing that the cost is evaluated starting from 1, avoiding to consider the feedback $\gamma(0)$.

Similarly, the other contributions can be discretized as:
\begin{IEEEeqnarray}{RCL}
\eqref{c6eq:cost_gamma2}{+}\eqref{c6eq:cost_gamma_ter} &\Rightarrow&  \Gamma_\gamma^{imp} = \nonumber\\
	 &=&\frac{1}{2}\sum_{k=\bar{k}_{imp}}^{N} \norm{\gamma(k) - \gamma^d(k)}^2_{K_\gamma^{imp}},
 \IEEEyessubnumber\\
\eqref{c6eq:cost_f} &\Rightarrow& \Gamma_f = \frac{1}{2}\sum_{k=0}^{N-1} \norm {f(k)}^2_{K_f} \IEEEyessubnumber,\\
\eqref{c6eq:cost_icp} &\Rightarrow& \Gamma_{icp}  {=}\frac{1}{2}\sum_{k=\bar{k}_{imp}}^{N} \norm{ x_{icp}(k) - x_{icp}^d(k)}^2_{K_{icp}} \IEEEyessubnumber
\end{IEEEeqnarray}
where $\bar{k}_{imp}$ is the minimum between $N$ and $k_{impact}$, so that $\Gamma_\gamma^{imp}$ is composed by at least one term, as if there were a terminal cost like in ${\Gamma}$. On the other hand, there is no terminal cost associated to $r_{icp}$ when the step does not happen in the horizon, therefore $\bar{k}_{icp}$ is the minimum between $N+1$ and $k_{impact}$.

We can exploit the simple structure of the cost function to further weight the difference of desired reaction forces between two subsequent time-steps. 
This new cost term in the discrete case has the following form:
\begin{equation}
\Gamma_{df} = \frac{1}{2}\sum_{0}^{k_{hor}-1} \norm {f(k)-f(k-1)}^2_{K_{df}} 
\end{equation}
with $K_{df}$ a suitable positive semi-definite matrix of gains and initialized with $f(-1)$, considered considered as a datum, e.g. it corresponds to the wrench necessary to satisfy the equilibrium of the robot momentum.

Finally, the overall cost function $\Gamma$ is:
\begin{equation}
\Gamma = \Gamma_\gamma + \Gamma_\gamma^{imp} + \Gamma_f +\Gamma_{icp} +\Gamma_{df}.
\end{equation}

%\subsubsection{Cost Function Transcription}
%Starting from a cost in the form 
%\begin{equation*}
%\Gamma_x = \frac{1}{2} \norm{a(x)-b}^2_K
%\end{equation*}
%with optimization variable $x$, it is possible to rewrite it as 
%\begin{equation*}
%\Gamma_x = \frac{1}{2} a(x)^\top K a(x) - a(x)^\top Kb + \frac{1}{2} b^\top K b.
%\end{equation*}
%The term $1/2 \: b^\top K b$ does not depend on $x$ and thus it can be ignored in the optimization problem. $H \equiv K$ is the Hessian and $\mathbbm{g} \equiv -K\;b$ the gradient.
%
%From now on, we will define the Hessian and the gradient associated with each contribution using the same subscripts of the corresponding $\Gamma_{(\cdot)}$. For example, $\Gamma_\gamma$ corresponds to:
%\begin{equation*}
%\Gamma_\gamma \Rightarrow H_\gamma + \mathbbm{g}_\gamma 
%\end{equation*}
%where 
%\begin{equation*}
%H_\gamma = E_\gamma^\top \underbrace{\begin{bmatrix}
%								K_\gamma & 0_{9\times 9} & \cdots & \\
%								0_{9\times 9} & K_\gamma & 0_{9\times 9} & \cdots\\
%								\vdots& & \ddots&\\
%								0_{9\times 9}& \cdots&&K_\gamma								 
%						 \end{bmatrix}}_{\in \: \mathbb{R}^{9N\times 9N}}E_\gamma
%\end{equation*}
%and
%\begin{equation*}
%\mathbbm{g}_\gamma = -E_\gamma^\top \begin{bmatrix}
%										K_\gamma & 0_{9\times 9} & \cdots & \\
%										0_{9\times 9} & K_\gamma & 0_{9\times 9} & \cdots\\
%										\vdots& & \ddots&\\
%										0_{9\times 9}& \cdots&&K_\gamma
%									\end{bmatrix}\begin{bmatrix}
%									\gamma^d(1)\\
%									\gamma^d(2)\\
%									\vdots\\
%									\gamma^d(N)
%									\end{bmatrix}
%\end{equation*}
%with 
%\begin{equation*}
%E_\gamma = \begin{bmatrix}
% {1}_{9} & 0_{9\times 9} & \cdots & 0_{9\times 9}&0_{9\times 12N} \\
%  0_{9\times 9} & {1}_{9}&\cdots & 0_{9\times 9}&0_{9\times 12N}\\
%\vdots&  &  \ddots   &   & \vdots\\
%0_{9\times 9} & \cdots & 0_{9\times 9} & {1}_{9}&0_{9\times 12N} 
%\end{bmatrix}.
%\end{equation*}
%The summation has been expanded by repeating the matrix of gains over the diagonal, while $E_\gamma \in \mathbb{R}^{9N\times 21N}$, similarly to what have been done in the constraints transcription, extracts the $\gamma$ terms from the vector $\chi$. $H_\gamma^{imp}$ and $\mathbbm{g}_\gamma^{imp}$ are obtained in the very same way, with the only difference that $K_\gamma$ is substituted by $K_\gamma^{imp}$ for all the positions corresponding to a $k\geq \bar{k}_{imp}$ and with a null matrix otherwise. 
%
%
%For what concerns the cost related to the control variable (the desired wrenches) $f$, a similar procedure has been performed:
%\begin{equation*}
%H_f = E_f^\top \underbrace{\begin{bmatrix}
%	K_f & 0_{12\times 12} & \cdots & \\
%	0_{12\times 12} & K_f & 0_{12\times 12} & \cdots\\
%	\vdots& & \ddots&\\
%	0_{12\times 12}& \cdots&&K_f								 
%	\end{bmatrix}}_{\in \: \mathbb{R}^{12N\times 12N}}E_f
%\end{equation*}
%with no gradient $\mathbbm{g}_f$ since the vector of desired wrenches is zero, while $E_f$ is the same matrix used in the transcription of constraints related to wrenches, defined in Eq. \eqref{c6eq:EFdef}. About the ``differential cost'' $\Gamma_{df}$ instead,
%\begin{equation*}
%H_{df} = E_f^\top F_{dif}^\top \underbrace{\begin{bmatrix}
%	K_{df} & 0_{12\times 12} & \cdots & \\
%	0_{12\times 12} & K_{df} & 0_{12\times 12} & \cdots\\
%	\vdots& & \ddots&\\
%	0_{12\times 12}& \cdots&&K_{df}								 
%	\end{bmatrix}}_{\in \: \mathbb{R}^{12N\times 12N}} F_{dif} E_f
%\end{equation*}
%with
%\begin{equation*}
%\mathbbm{g}_{df} = -E_f^\top F_{dif}^\top \begin{bmatrix}
%	K_{df} & 0_{12\times 12} & \cdots & \\
%	0_{12\times 12} & K_{df} & 0_{12\times 12} & \cdots\\
%	\vdots& & \ddots&\\
%	0_{12\times 12}& \cdots&&K_{df}								 
%	\end{bmatrix}\begin{bmatrix}
%					f(-1)\\
%				    0_{12}\\
%					\vdots\\
%					0_{12}
%					\end{bmatrix}
%\end{equation*}
%where $f(-1)$ is considered as given (as discussed above) and $F_{dif}$ selects the correct wrenches with the right sign, i.e.
%\begin{equation*}
%F_{dif} = \begin{bmatrix}
%1_{12} & 0_{12\times 12} &\cdots & &0_{12\times 12}\\
%-1_{12}& 1_{12} & 0_{12\times 12} &\cdots & \\
%0_{12\times 12} &-1_{12}& 1_{12} & 0_{12\times 12} &\cdots\\
%\vdots & & \ddots & \ddots&\\
%0_{12\times 12} & \cdots && -1_{12}& 1_{12}
%\end{bmatrix}.
%\end{equation*}
%Finally, for what concerns the ICP related cost,
%\begin{equation*}
%H_{icp} = E_{\gamma}^{k_{2f}\top} E_{icp}^\top \begin{bmatrix}
%	K_{icp} & 0_{2\times 2} & \cdots & \\
%	0_{2\times 2} & K_{icp} & 0_{2\times 2} & \cdots\\
%	\vdots& & \ddots&\\
%	0_{2\times 2}& \cdots&&K_{icp}								 
%	\end{bmatrix}E_{icp} E_{\gamma}^{k_{2f}} 
%\end{equation*}
%while 
%\begin{equation*}
%\mathbbm{g}_{icp} =  E_{\gamma}^{k_{2f}\top} E_{icp}^\top 
%\begin{bmatrix}
%K_{icp} &  \cdots & 0_{2\times 2} \\
%\vdots&  \ddots&\\
%0_{2\times 2}& \cdots&K_{icp}								 
%\end{bmatrix}\begin{bmatrix}
%r_{icp}^d(k_{impact}+1)\\
%r_{icp}^d(k_{impact}+2)\\
%\vdots\\
%r_{icp}^d(N)
%\end{bmatrix}
%\end{equation*}
%where the gain matrix $K_{icp}$ has been repeated $N-k_{impact}+1$ times, supposing to have $k_{impact}$ inside the horizon, otherwise $H_{icp}$ and $\mathbbm{g}_{icp}$ simply disappear.
%
%Finally, the Hessian and the gradient of Eq. \eqref{c6eq:optim_cost} take the following expression:
%\begin{IEEEeqnarray}{RCL}
%	\IEEEyesnumber \phantomsection
%	H &=& H_\gamma + H_\gamma^{imp} + H_f + H_{df} + H_{icp} \IEEEyessubnumber\\
%	\mathbbm{g} &=& \mathbbm{g}_\gamma + \mathbbm{g}_\gamma^{imp} + \mathbbm{g}_{df} + \mathbbm{g}_{icp} \IEEEyessubnumber
%\end{IEEEeqnarray}
%
%In order to solve the optimization problem described in \eqref{c6eq:optim}, we decided to adopt the ``interior point method'' which happened, in our application, to be orders of magnitude faster than ``active set'' algorithms, as suggested in \cite{bartlett2000active}. This may be mainly due to the very sparse structure of the problem.

